Achieving an Efficient and Fair Equilibrium Through Taxation

It is well known that a game equilibrium can be far from efficient or fair, due to the misalignment between individual and social objectives. The focus of this paper is to design a new mechanism framework that induces an efficient and fair equilibrium in a general class of games. To achieve this goal, we propose a taxation framework, which first imposes a tax on each player based on the perceived payoff (income), and then redistributes the collected tax to other players properly. By turning the tax rate, this framework spans the continuum space between strategic interactions (of selfish players) and altruistic interactions (of unselfish players), hence provides rich modeling possibilities. The key challenge in the design of this framework is the proper taxing rule (i.e., the tax exemption and tax rate) that induces the desired equilibrium in a wide range of games. First, we propose a flat tax rate (i.e., a single tax rate for all players), which is necessary and sufficient for achieving an efficient equilibrium in any static strategic game with common knowledge. Then, we provide several tax exemption rules that achieve some typical fairness criterions (such as the Max-min fairness) at the equilibrium. We further illustrate the implementation of the framework in the game of Prisoners' Dilemma.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> app-mcs-edge.tex <==

\subsubsection{Problem Formulation}


Now we formulate the task selection (and order) problem for each user.
As shown in Figure \ref{fig:mcs-model}, the task selection (and order) of each user can be characterized by a \emph{single-path route}, initiating from the user's initial location and passing through the selected tasks in a given order.
In the example of Figure \ref{fig:mcs-model}, the task selection (and order) of user $1$ can be captured by the route $\widetilde{1}\rightarrow 1 \rightarrow 2 \rightarrow 3 \rightarrow 4$, where $\widetilde{1} $ denotes the user index.
It is important to note that given the task selection, there can be multiple routes (task orders). For example, user $1$ can also execute task $2$ first, and then task $1$ in the  above example.
This is the key difference of our model with that in \cite{xxx-4}, where the route (task order) is given as long as the tasks are selected (as each task is associated with a specific time  \cite{xxx-4}).
This introduces additional challenge in our task selection problem formulation.

We resolve this challenge by transferring the task selection and order problem into an \emph{edge selection} problem.
The key idea is that each task selection and order can be captured by a route, which can be further characterized by a set of edges.
In the example of Figure \ref{fig:mcs-model}, the route $\widetilde{1} \rightarrow 1 \rightarrow 2 \rightarrow 3 \rightarrow 4$ can be characterized by a set of directed edges:
$e_{\widetilde{1}\rightarrow 1}$,
$e_{1\rightarrow 2}$,
$e_{2\rightarrow 3}$,
and
$e_{3\rightarrow 4}$.
Therefore, the task selection and order of each  user $i$ can be characterized by a proper selection of edges among himself and all tasks: \emph{the tasks in the selected edges denote the task selection and the direction of each edge denote the order of the associated tasks}.


\emph{(a) Route Feasibility.}
Let $x_{k \rightarrow k'}^{(i)} \in \{0, 1\}$ denote whether the edge between nodes $k $ and $ k' $ is selected by user $i$, where $k, k' \in \S \bigcup \{\widetilde{i}\}$.
Since a feasible route is continue and single-path, we have the following  constraint: (i) for each node $k' \in \S \bigcup \{\widetilde{i}\} $, its incoming edge cannot be more than $1$, i.e.,
\begin{equation}\label{eq:route-1}
\sum_{k \in \S \bigcup \{\widetilde{i}\} } x_{k \rightarrow k'}^{(i)} \leq 1
, \quad \forall k' \in \S \bigcup \{\widetilde{i}\};
\end{equation}
(ii) for each node $k' \in \S \bigcup \{\widetilde{i} \}$, its outgoing edge  cannot be more than $1$, i.e.,
\begin{equation}\label{eq:route-2}
\sum_{k \in \S \bigcup \{\widetilde{i}\} } x_{k' \rightarrow k}^{(i)} \leq 1
, \quad \forall k' \in \S \bigcup \{\widetilde{i}\};
\end{equation}
and (iii) for each task node $k' \in \S $, if there exists an outgoing edge, there must be an incoming edge, i.e.,
\begin{equation}\label{eq:route-3}
\sum_{k \in \S \bigcup \{\widetilde{i}\} } x_{k' \rightarrow k}^{(i)} \leq \sum_{k \in \S \bigcup \{\widetilde{i}\} } x_{k \rightarrow k'}^{(i)}
, \quad \forall k' \in \S .
\end{equation}
Note that   constraint \eqref{eq:route-3} is not required for the user node $\{\widetilde{i}\} $, as it is the initial node of each route.

Recall that the tasks in the selected edges denote the selected tasks.
Let $z_{k}^{(i)} \in \{0, 1\}$ denote whether a task $k \in \S$ is selected (executed) by user $i$. Then,
\begin{equation}\label{eq:route-4}
z_{k}^{(i)} = \sum_{k' \in \S \bigcup \{\widetilde{i}\} } x_{k' \rightarrow k}^{(i)}.
\end{equation}


We further note that a feasible route is acyclic (i.e., no cycle), which can be achieved by the following time constraint:
the executing time of the task in the downstream of an edge must be later than that of the task in the upstream of the edge.
In the example of Figure \ref{fig:mcs-model}, the executing time of task $1$ is later than that of task $2$ by user $1$.
Let $T_{k}^{(i)} \geq 0$ denote the executing time of task $ k \in \S $ by user $i$. Formally,
\begin{equation}\label{eq:route-5}
T_{k}^{(i)} \geq T_{k'}^{(i)} + \frac{D(L_k, L_{k'})}{r_i}, \quad \mbox{if~~} x_{k' \rightarrow k}^{(i)} = 1,
\end{equation}
where $D(L_k, L_{k'}) $ denotes the distance between $k$ and $k'$.
Note that the above constraint can remove any cycle in the route. Suppose there exists a cycle $k_1 \rightarrow k_2 \rightarrow k_3 \rightarrow k_1$ in a route. Then, by the above constraint, we have: $T_{k_2}^{(i)} > T_{k_1}^{(i)}$, $T_{k_3}^{(i)} > T_{k_2}^{(i)}$, and $T_{k_1}^{(i)} > T_{k_3}^{(i)}$,  which lead to contradiction.



\emph{(b) Task Time Sensitivity.}
Recall that each task $k$ is associated with a valid time period $T_k \eq [ T_k^{\textsc{s}},T_k^{\textsc{e}} ]$, within which the task must be executed.
Thus, we have the following time sensitivity constraint for each task $k \in \S$:
\begin{equation}\label{eq:route-6}
 T_k^{\textsc{s}} \leq T_{k}^{(i)} \leq T_k^{\textsc{e}},
\end{equation}
for any task $k\in\S$ selected by user $i$, i.e., $z_{k}^{(i)}=1$.

\emph{(c) User Budget Constraint.}
Recall that each user $i$ has a limited resource $C_i$ for executing tasks.
Thus, we have the following budget constraint for each user $i \in \N$:
\begin{equation} \label{eq:route-7}
\sum_{k \in \S}  c_{i, k} \cdot z_{k}^{(i)}  \leq C_i .
\end{equation}

\vspace{2mm}

Let $\bx_i \eq ( x_{k \rightarrow k'}^{(i)}, \forall k, k' \in \S \bigcup \{\widetilde{i}\} ) $ denote a feasible edge selection of user $i$. Then the difference between
the total reward and the executing cost of user $i$  is
\begin{equation}
\sum_{k\in\S} z_{k}^{(i)} \cdot \left( \frac{w_k}{M_k } - c_{i,k} \right),
\end{equation}
where $M_k = \sum_{i\in\N} z_{k}^{(i)} $  denotes the number of users selecting task $k$.
The total moving cost that user $i$ incurs is
\begin{equation}
 \sum_{k \in \S \bigcup \{\widetilde{i}\} } \sum_{k' \in \S \bigcup \{\widetilde{i}\} }
  x_{k \rightarrow k'}^{(i)} \cdot  Dis(L_k, L_{k'}) \cdot \widetilde{c}_i.
\end{equation}
Thus, the total payoff of each user $i$ is as follows:
\begin{equation}
\begin{aligned}
u_i(\bx_i) \eq &  \sum_{k\in\S} z_{k}^{(i)} \cdot \left( \frac{w_k}{M_k } - c_{i,k} \right)
\\
 & - \sum_{k \in \S \bigcup \{\widetilde{i}\} } \sum_{k' \in \S \bigcup \{\widetilde{i}\} }
  x_{k \rightarrow k'}^{(i)} \cdot  Dis(L_k, L_{k'}) \cdot \widetilde{c}_i .
\end{aligned}
\end{equation}


Therefore, the task selection problem of each user $i \in \S$ can be written as follows:
\begin{equation}
\begin{aligned}
\max_{\bx_i} \ & \  u_i(\bx_i)
\\
\mbox{s.t.}  \ & \eqref{eq:route-1}\sim\eqref{eq:route-7}
\end{aligned}
\end{equation}
Note that the payoff $u_i (\bx_i)$ of user $i$ also depends on the other users' edge selections $\bx_{i'}, \forall i' \neq i$, as   $M_k$ depends on other users' choices.
As shown in \cite{xxx-4}, a simplified version of the task selection problem in \cite{xxx-4} is NP-hard. Our problem is much more challenging than that in \cite{xxx-4}, as we need to consider not only the task selection but also the task order.
Even given the task selection, the task order optimization is still an NP-hard problem.

In order to obtain more useful engineering insights, we consider a simplified model for the  implementation and evaluation of the proposed Taxation Mechanism.\footnote{The complete analysis for the original model can be found in our online technical report \cite{report}.}
In the simplified model, we assume that (i) each task is valid in the whole time period, and (ii) each user has a zero moving cost.
With the above model simplifications, the choice of each user is to choose a set of available tasks to execute, where the task order is not required.

\comm{We have formulated a general problem, but later on we focus on a much simpler setting. If we do not come back to the more general problem (for example, through numerical study), then a reader might feel that we are "over-claiming" the problem (as formulating a complicated problem without solving it is not a major contribution).
\\
More specifically, since we consider a much simpler problem from now on, our analysis and later simulation do not provide new insights comparing with [38] (in terms of the MCS literature).
\\
We need to think about this issue very carefully. }



==> app-mcs-simu.tex <==


\begin{figure}
	\centering
\includegraphics[width=3.5in]{Figures/MCS-simu-map}
	\caption{Illustration of A 5km$\times$5km Simulation Region in London. Triangle: Tasks; Circle: Users.}
\label{fig:mcs-simu-map}
\end{figure}

In this subsection, we provide additional simulation results for the more general and practical scenarios.

\subsubsection{Simulation Setting}
As shown in Figure \ref{fig:mcs-simu-map}, we choose a 5km$\times$5km region in London as the simulation area.
Tasks and users are randomly and uniformly distributed within the simulation area.
We simulate the task selection and execution in a period of $2$ hours, e.g., [10:00, 12:00].
Each task is initiated within the 2-hour simulation period randomly and uniformly, and the task valid (survival) time is selected randomly according to the (truncated) normal distribution with the expected value of $30$ minutes.
Each task needs to be executed (but not necessarily to be completed) within its valid time period.
The reward of each task is selected randomly according to  the (truncated) normal distribution with the expected value of $\$10$ (in dollar).

We consider three types of different users according to their travelling modes: (i) \emph{Walking users}, who travel by walking, with a relatively low travelling speed and cost; (ii) \emph{Bike users}, who travel by bike, with a medium travelling speed and cost, and (iii) \emph{Driving users}, who travel by driving, with a relatively high travelling speed and cost.
We set the travelling speed and cost for each user randomly according to the (truncated) normal distribution, with the expected values of (i) $5$km/h  and $\$0.2$/km for walking users, (ii) $15$km/h  and $\$0.5$/km for bike users, and (iii) $45$km/h  and $\$1$/km for driving users.
Moreover, each user takes on average $10$ minutes to execute a task, incurring an execution cost of $\$1$ (in dollar) on average.
Both the execution time and cost follow the (truncated) normal distribution as other parameters.

In the simulations, we fix the number of tasks by $8$, while change the number of users from $2$ to $20$ (to capture different levels of competition among users).
For each scenario (with a particular user type and number), we run 1000 simulations and take the average results.



\subsubsection{Social Welfare Gain}
We first show the social welfare gain achieved by our proposed Taxation Mechanism.

Figure \ref{fig:mcs-simu-sw} illustrates the expected social welfare under SE and NE with three different types of users.
Note that the SE is induced by our proposed Taxation Mechanism, while the NE is achieved in the original game situation without the Taxation Mechanism.
Hence, the social welfare gap between the SE and the NE can be viewed as the social welfare gain achieved by our proposed Taxation Mechanism.
In the first subfigure (a), all the users are walking users with low travelling speed and cost.
In the second subfigure (b), all the users are bike users with medium travelling speed and cost.
In the third subfigure (c), all the users are driving users with high travelling speed and cost.

From Figure \ref{fig:mcs-simu-sw}, we can see that the social welfare under SE increases with the number of users in all three scenarios (walking users, bike users, and driving users).
This is because with more users, it is more likely the tasks can be executed by lower cost users, hence resulting in a higher social welfare.
We can further see that the social welfare under NE decreases with the number of users in most cases.
This is because from the individual perspective,  with more users, the competition among users becomes more intensive, and the probability that multiple users choosing the same task increases, which will lead to a higher execution/travelling cost and hence a lower social welfare.
We also note that in the scenario (a) with walking users, when the number of walking user is small (e.g., less than 5), the social welfare under NE  increases with the number of users slightly.
This is because the walking users often have a limited serving region due to the small travelling speed, hence, there is almost no competition among users when the number of users is small.
In this case, increasing the number of users will not introduce much competition among users, but will increase the probability that the tasks being executed by lower cost users, hence resulting in a higher social welfare.
This coincides with the numerical results in Figure \ref{fig:simu-1}, where the social welfare under NE  increases with the number of users when the user number is small.

Similar as the numerical results in Figure \ref{fig:simu-1}, the simulation results in Figure \ref{fig:mcs-simu-sw} also indicate that with our proposed Taxation Mechanism (that leads to the  SE), it is always beneficial (for social welfare) to involve more users in the system; while without the proposed Taxation Mechanism (leading to the NE), it is often harmful (for social welfare) to involve more users, due to the increased competition among users.
In this sense, our proposed Taxation Mechanism can reconcile the competition among users and align the individual objectives with the social objective, hence reach the desired efficient equilibrium.

Figure \ref{fig:mcs-simu-ratio} presents the ratio of social welfare under SE and NE with three different types of users.
As mentioned previously, such a social welfare ratio between the SE and the NE can be viewed as the performance gain achieved by our proposed Taxation Mechanism.
From Figure \ref{fig:mcs-simu-ratio}, we can see that in all three scenarios, the social welfare ratio increases with the number of users.
This is because the social welfare increases with the number of users under SE , while  (mostly) decreases with the number of users under NE, as illustrated in the previous Figure \ref{fig:mcs-simu-sw}.
We can further see that the social welfare ratio with walking users is lower than those with bike users and driving users.
This is because the competition among walking users is less intensive than that among bike/driving users, due to the limited traveling speed and serving region of walking users.
Hence, the degradation of social welfare under NE (comparing with SE) is smaller with walking users.
More specifically, we can find from Figure \ref{fig:mcs-simu-ratio}  that when the number of users is $20$,  the social welfare ratio can be up to $270\%$, $330\%$, and $280\%$ for walking users, bike users, and driving users, respectively.

\begin{figure}
	\centering
\includegraphics[width=3.2in]{Figures/MCS-simu-ratio}
	\caption{Ratio of Social Welfare between SE and NE.}
\label{fig:mcs-simu-ratio}
\end{figure}



\subsubsection{Average Number of Users per Task}
We now show the average number of users choosing a task.
Note that the performance degradation under NE (comparing with SE) is mainly due to the  possibility of multiple users choosing the same task (especially when the reward of the task is large). This will cause certain system performance loss, as from the social perspective, one user is sufficient for each task.
In general, a higher number of users per task will lead to a larger performance loss.

Figure \ref{fig:mcs-simu-zk} illustrates the average number of users per task under SE and NE.
We can see that under SE, the average number of users per task is always $1$.
This is because under SE, none of the task will be selected by multiple than one user; otherwise, if a task is selected by multiple users, the social welfare can be immediately improved by removing all users except one in the task.
We can further see that under NE, the average number of users per task increases with the total  number of users, and can be up to $6$, $5$, and $4$ (for walking users, bike users, and driving users, respectively) when the total number of users is 20.
This implies that a larger number of users will lead to a more intensive competition among users and result in a larger social welfare performance degradation as shown in the previous Figure \ref{fig:mcs-simu-sw}

\begin{figure}
	\centering
\includegraphics[width=3.1in]{Figures/MCS-simu-zk}
	\caption{Average Number of Users per Task under SE and NE.}
\label{fig:mcs-simu-zk}
\end{figure}


\subsubsection{Fairness}
We now show the fairness achieved by our proposed Taxation Mechanism, which captures how the generated social welfare is distributed among users.

We evaluate the fairness by the widely-used Jain's fairness index, which is defined as follows:\footnote{For more details, please refer to the report DEC-TR-301 in Eastern Research Lab: ``A quantitative
measure of fairness and discrimination for resource
allocation in shared computer systems'' written by R. K. Jain, D. Chiu, and W. R. Hawe in 1984.}
$$
J(\bs) = \frac{\left( \sum_{i\in\N} \u_i(\bs) \right)^2}{N \cdot \sum_{i\in\N} \u_i(\bs)^2  } .
$$
By the above definition, it is easy to see that the maximum Jain's fairness is $1$, which can be achieved when all users share the social welfare equally, and the minimum Jain's fairness is $\frac{1}{N}$, which can be achieved when one user gets all of the social welfare while all other users get a zero payoff.

Figure \ref{fig:mcs-simu-jane} illustrates the Jain's fairness index under SE (achieved by our proposed Taxation Mechanism with the identical tax exemption for all users) and NE (achieved in the original game situation without the Taxation Mechanism).
We can see that under SE (achieved by our proposed Taxation Mechanism with the identical tax exemption), we can always achieve the maximum Jain's fairness index $1$.
This is because with our proposed Taxation Mechanism (together with the identical tax exemption), all the users will share the generated social welfare equally according to Lemma \ref{lemma:fair1}, hence resulting in the maximum Jain's fairness $1$.
We can further see that under NE (without our proposed Taxation Mechanism), the Jain's fairness index decreases with the number of users, and can be down to $0.8$, $0.6$, and $0.5$ (for walking users, bike users, and driving users, respectively) when the total number of users is 20. This implies that a larger number of users will lead to a poor fairness under NE.
This is because a larger number of users will lead to a more intensive competition among users, hence it is more likely that some highly competitive users occupy most of the social welfare, resulting in a lower fairness index.

Figure \ref{fig:mcs-simu-jane} also shows that under NE (without our proposed Taxation Mechanism), the Jain's fairness index with walking users is often higher than those with bike users and driving users.
This is because the competition among walking users is less intensive than that among bike or driving users, due to the limited traveling speed and serving region of walking users.
Thus, with bike or driving users, it is more likely that some highly competitive users occupy most of the social welfare, resulting in a lower fairness index.


\begin{figure}
	\centering
\includegraphics[width=3.15in]{Figures/MCS-simu-Jane}
	\caption{Jane's Fairness Index under SE and NE.}
\label{fig:mcs-simu-jane}
\end{figure}


==> app-mcwa.tex <==

%\subsection{Analysis for Application II -- MCWA}\label{app:9}


%Mobile Crowdsourced Wireless Access (MCWA) enables nearby mobile devices to form a cooperative group (via D2D communication technology such as WiFi or Bluetooth) and  crowdsource their wireless access channels and resources
%for the  cooperative data downloading and uploading \cite{yyy-1}.
%Such a novel networking scheme reconciles the mismatch between mobile users' data demands and their wireless access capacities,
%hence can achieve a more efficiently utilization of wireless resources.

In this application, we will formulate a \emph{Channel Selection Game} for a basic MCWA model similar as that in \cite{yyy-1},
and show how to implement the Taxation Mechanism in this game, and how the Taxation Mechanism will steer the
results of the Channel Selection Game to a desirable one.
%Due to space limit, we leave the detailed discussion in our online technical report \cite{report}.
Next, we provide the detailed discussions for this model.

\subsubsection{System Model}

We consider a set $\N = \{1,\cdots,N\}$ of $N$ nearby mobile users, each connecting to a base station to access the Internet.
Let $\S_i$ denote the set of available channels that each user $i \in \N $ can operate on (for connecting to his base station),
and $\S \eq \bigcup_{i\in\N} \S_i $ denote the set of all available channels of all users.
An available channel for a user can be an orthogonal code (in a CDMA system) or a set of orthogonal sub-carrier frequencies (in an OFDMA system) that the base station assigns to the user.
Thus, there is no mutual interference between different channels.

Each user can choose to operate on one or multiple available channels.
Moreover, each user needs to select a transmission power level for each operating channel that he chooses, under a given power budget.
%Let $\bs_i \subseteq \S_i$ denote the set of operating channels that user $i $ chooses, and
%$\bp_i \eq \{ \p_i(k), \forall k\in \bs_i \}$ denote the transmission power levels for all chosen channels, where $ \sum_{k\in \bs_i} \p_i(k) \leq P_i $, and $P_i$ the power budget of user $i$.
The transmission of a user on a chosen channel will interfere and be interfered by the transmissions of other users on the same channel.
The \emph{payoff} of each user is defined as the total channel capacity that he achieves on all chosen channels under the given power budget.

For convenience, we list the key notations used in the following discussion as follows.
\begin{itemize}
  \item $\bs_i \subseteq \S_i$: the set of operating channels that user $i $ chooses;
  \item $\bp_i \eq \{ \p_i(k), \forall k\in \bs_i \}$: the transmission power levels that user $i$ selects for his operating channels.
        For notational convenience, we will deote $p_i(k) \equiv  0$ for all $ k \notin \bs_i$ (i.e., those channels not chosen by user $i$);
  \item $g_{ii}(k) \geq 0 $: the gain of channel $k$ between user $i$ and his base station (i.e., transmission channel gain);
  \item $g_{ji}(k) \geq 0 $: the gain of channel $k$ between user $i$ and user $j$'s base station (i.e., interference channel gain);
\end{itemize}


\subsubsection{Game Formulation}
The strategy of each user $i \in \N$ is to choose a subset $\bs_i \subseteq \S_i $ of operating channels and the corresponding power levels $\bp_i$, aiming at maximizing his payoff, considering his power budget constraint: $ \sum_{k\in \bs_i} \p_i(k) \leq P_i $, where $P_i$ is the power budget of user $i$.

Given the strategy profile $(\bs, \bp) = (\bs_1,\cdots,\bs_N,\bp_1, \cdots,$ $\bp_N)$, i.e., the channel and power selections of all users, the payoff (total capacity) of each user $i \in \N $ is given by the well-known Shannon-Hartley theorem in information theory:\footnote{For more details, please refer to ``The Mathematical Theory of Communication'' written by C.E.~Shannon in 1949.}
\begin{equation}\label{eq:yyy:payoff}
\u_i (\bs,\bp) =
\sum_{k \in \bs_i} B_k \log \left(1 + \frac{g_{ii}(k)   \p_i(k) }{ \sigma_k + \sum_{j\neq i} g_{ij}(k)   \p_j(k) } \right),
\end{equation}
where $B_k$ is the bandwidth of channel $k  $, $\sigma_k$ is the average noise power on channel $k$, and $\sum_{j\neq i} g_{ij}(k) \p_j(k)$ is the total interference power on channel $k$ from all other users.
% Note that $p_j(k) \equiv  0 $ when $k \notin \bs_j$, i.e., user $j$ doesn't choose channel $k$.
For  notational convenience, we will also write $\u_i (\bs,\bp) $ as $\u_i (\bs_i , \bs_{-i}, \bp_i, \bp_{-i})$,
where
$(\bs_{-i} , \bp_{-i} ) \eq  ( \bs_1,\cdots,\bs_{i-1}, \bs_{i+1},$ $\cdots,\bs_N,\bp_1,\cdots,\bp_{i-1},\bp_{i+1},\cdots, \bp_N )$ is the strategy profile of all other users except $i$.


Based on the above discussion, we can formally define the Channel Selection Game and the associated NE as follows.
\begin{definition}[Channel Selection Game]\label{def:channel-game}
A Channel Selection Game, denoted by $\C \eq (\N, \{\S_i \}_{i\in\N}, \{\u_i\}_{i\in\N})$, is given by:
\begin{itemize}
  \item  \textbf{Player}: a set $\N = \{1, \cdots , N\}$ of nearby mobile users;
  \item  \textbf{Strategy}: a set of available channels $\S_i$ for each user $i$;
  \item  \textbf{Payoff}: a payoff function   $ \u_i (\bs, \bp)$   in \eqref{eq:yyy:payoff} for each user~$i $.
\end{itemize}
\end{definition}


A strategy profile $(\bs^*,\bp^* ) \eq (\bs_1^*,\cdots,\bs_N^*, \bp_1^*,\cdots,\bp_N^*)$ is an NE of the game $\C$, if for every user $i\in\N$,
\begin{equation}\label{eq:yyy:ne}
\begin{aligned}
 (\bs_i^*, \bp_i^*) = \arg \max_{\bs_i \subseteq \S_i, \bp_i \succeq \boldsymbol{0}} & \   \u_i (\bs_i, \bs_{-i}^*, \bp_i, \bp_{-i}^*)
 \\
  s.t.\ & \sum_{k\in \bs_i} \p_i(k) \leq P_i
\end{aligned}
\end{equation}
That is, the strategy $ (\bs_i^*, \bp_i^*) $ of each user $i $ in an NE is his best response to the strategies $  (\bs_{-i}^*, \bp_{-i}^*) $ of other players.
%Hence, no user has the incentive to   unilaterally deviate from  $\bs^* $.



\subsubsection{Equilibrium Analysis}
We now analyze the NE of the Channel Selection Game $\C$ \emph{without} the Taxation Mechanism, and show that the corresponding NE is often \emph{not} efficient.

By \eqref{eq:yyy:payoff}, we can easily find that each user's best strategy is to use all of his power budget (on his chosen channels), no matter what strategies that other users choose. Formally,
\begin{lemma} \label{lemma:yyy:1}
If $(\bs^*, \bp^* )$ is an NE of the game $\C$, then
 \begin{equation}\label{eq:yyy:ne1}
  \sum_{k\in \bs_i^*} \p_i^*(k) = P_i,\quad \forall i\in\N.
 \end{equation}
\end{lemma}

\begin{proof}
The proof is straightforward: if $\sum_{k\in \bs_i^*} \p_i^*(k) < P_i$ for a user $i$, then he can directly increase his payoff by assigning the remaining power budget to any of his chosen channels.
\end{proof}

We can further see that given the strategy profile $  (\bs_{-i}^*, \bp_{-i}^*) $ of other users, the best channel selection and power allocation of   user $i$ follows the water-filling principle. Formally,
\begin{lemma}\label{lemma:yyy:2}
If $(\bs^*, \bp^* )$ is an NE of the game $\C$, then the equilibrium strategy $(\bs_i^*, \bp_i^* )$ of each user $i \in \N$ satisfies:~~~~~~~~~~~~
 \begin{equation}\label{eq:yyy:ne2a}
  \p_i^*(k) = \left[ \frac{B_k}{\lambda_i^*} - \frac{I_i^*(k)}{ g_{ii}(k) } \right]^+,\quad \forall k\in \S_i,
 \end{equation}
and
 \begin{equation}\label{eq:yyy:ne2b}
 \bs_i^* = \{k \ |\ k \in \S_i, \p_i^*(k)>0 \}, ~~~~~~~~~~
\end{equation}
 where $[x]^+ = \max(x,0)$,
 $I_i^*(k) \eq \sigma_k + \sum_{j\neq i} g_{ij}(k)  \p_j^*(k) $ is the noise and interference power on channel $k$ for user $i$, and $\lambda_i^*$ is the Lagrange multiplier for the power budget constraint.
\end{lemma}

\begin{proof}
By Lemma \ref{lemma:yyy:1}, we can rewrite the power budget constraint in \eqref{eq:yyy:ne} as
$ \sum_{k\in \bs_i } \p_i (k) = P_i $ for each user $i \in \N $.
Now let us solve the user decision problem \eqref{eq:yyy:ne} with the new power budget constraint.

Following the Lagrangian method, we introduce a Lagrange multiplier $\lambda_i$ for the new power budget constraint, and obtain the corresponding Lagrangian function:
$$
\L_i (\bs_i,  \bp_i) \eq \u_i (\bs_i, \bs_{-i}^*, \bp_i, \bp_{-i}^*) + \lambda_i \cdot \left( P_i  - \sum_{k\in \bs_i } \p_i (k)  \right).
$$
The partial derivative of $\L_i (\bs_i,  \bp_i)$ with respect to $\p_i (k)$ is:
\begin{equation}\label{eq:yyy:partial-ne}
\frac{\partial \L_i (\bs_i,  \bp_i) }{ \partial \p_i (k) } = B_k \cdot \frac{g_{ii}(k)  }{I_i^*(k) +  g_{ii}(k)   \p_i(k)   } - \lambda_i.
\end{equation}
By the KKT conditions, we can obtain the optimal solution:
$$
  \p_i^*(k) = \left[ \frac{B_k}{\lambda_i^*} - \frac{I_i^*(k)}{ g_{ii}(k) } \right]^+,\quad \forall k\in \S_i,
$$
where the optimal Lagrange multiplier $\lambda_i^*$ is given by
$$
  \sum_{k\in \S_i } \left[ \frac{B_k}{\lambda_i^* } - \frac{I_i^*(k)}{ g_{ii}(k) } \right]^+   = P_i .
$$
Intuitively, $ \frac{B_k}{\lambda_i^*} $ can be regarded as the water level for the power allocation of user $i$: increasing the water level (or reducing the Lagrange multiplier $\lambda_i^*$) will increase the power allocated to each chosen channel.

Moreover, when user $i$ allocates a zero power to a channel $k$ (i.e., $\p_i^*(k) = 0$), we can equivalently say that user $i$ does not choose channel $k$. Hence, the   optimal channel selection is given as follows: $ \bs_i^* = \{k \ |\ k \in \S_i, \p_i^*(k)>0 \}. $
\end{proof}

Lemma \ref{lemma:yyy:1} states that if there exists an NE $(\bs^*, \bp^* )$ for the game $\C$, then each user's equilibrium strategy under the NE must follow the water-filling principle given in \eqref{eq:yyy:ne2a} and \eqref{eq:yyy:ne2b}.
However, we can guarantee neither the uniqueness nor the existence of the NE of  the game $\C$.
Moreover, even if there exists an NE $(\bs^*, \bp^* )$, it can be far from efficient.

Specifically, a strategy profile $(\bs^\circ,\bp^\circ ) $ is socially efficient, if it maximizes the following social welfare:
\begin{equation}\label{eq:yyy:sw}
\W(\bs,\bp) =  \sum_{i \in \N} \sum_{k \in \bs_i} B_k \log \left(1 + \frac{g_{ii}(k)   \p_i(k) }{ \sigma_k + \sum_{j\neq i} g_{ij}(k)   \p_j(k) } \right),
\end{equation}
under the power budget constraints of all users, that is, $ \sum_{k\in \bs_i } \p_i (k) \leq P_i , \forall i
 \in \N$. The partial derivative of the social welfare $\W(\bs,\bp)$ with respect to $\p_i (k)$ is:
\begin{equation}\label{eq:yyy:partial-se}
\frac{\partial \W(\bs,\bp) }{ \partial \p_i (k) } = \frac{\partial \u_i(\bs,\bp) }{ \partial \p_i (k) }
+ \sum_{j\neq i} \frac{\partial \u_j(\bs,\bp) }{ \partial \p_i (k) } ,
\end{equation}
where $\frac{\partial \u_i(\bs,\bp) }{ \partial \p_i (k) } > 0 $
and $\frac{\partial \u_j(\bs,\bp) }{ \partial \p_i (k) } < 0, \forall j\neq i$.
The first term indicates  that user $i$ benefits from an increased transmission power on a channel $k$, while the second term indicates that all other users suffer from an increased transmission power of user $i$ on channel $k$.
This implies that from the social perspective, it is more conservative for a user to assign power to a channel, considering the potential interference to other users.

To illustrate this, we provide a simple example with one channel (denoted by $k$) and two users $i\in \{1,2\}$. Suppose that the transmission channel gains are $g_{11}(k) = g_{22}(k) = 1$, the interference channel gains  are $g_{12}(k) = g_{21}(k) = 1$, the power budgets are $P_1 = P_2 = 2$, and the average noise power is $\sigma_k = 0.2$.
The SE outcome is: only user 1 or 2 transmits with the maximum power, leading to a social welfare of $\log(1+\frac{2*1}{0.2})\approx 1.04$.
Under the NE, however, both users will transmit with the maximum power, leading to a social welfare of $2 \cdot \log(1+\frac{2*1}{0.2 + 2*1}) \approx 0.56$, an degradation of $50\%$ comparing with that in the SE.


\subsubsection{\textbf{Implementation of Taxation Mechanism}}

Now we implement the Taxation Mechanism in the Channel Selection Game $\C$ to induce the efficient and fair equilibrium.

For ease of illustration, we set  $\bg = 1$ (i.e., strictly budget balance) and $\ex_i = 0, \forall i\in \N$ (i.e., zero tax exemptions for all users, leading to the Max-min fairness by Lemma \ref{lemma:fair1}).
Then, according to Theorem \ref{thm:efficiency}, the efficient flat taxing rule is:
\begin{equation}
\r_i = \r = \frac{N-1}{N}, \quad \forall i \in \N.
\end{equation}
With the above taxing rule, the new payoff of each user $i\in \N$  in the Taxation Version of the game $\T$, according to  \eqref{eq:xxx}, can be computed as follows:
\begin{equation}\label{eq:yyy:payoff-tax}
\begin{aligned}
 \ux_i (\bs,\bp) &   =  \left(1 - \frac{N-1}{N}\right) \u_i(\bs,\bp) + \frac{N-1}{N}   \frac{1}{N-1}   \sum_{j\neq i}\u_j(\bs,\bp)
 \\
 &   = \frac{ 1}{N}  \cdot \u_i(\bs,\bp ) + \frac{ 1}{N}  \cdot \sum_{j \neq i } \u_j(\bs,\bp )
% \\
% &     =\frac{ 1}{N} \cdot \sum_{l \in \N} \sum_{k \in \bs_l} B_k \log \left(1 + \frac{g_{ll}(k)   \p_l(k) }{ \sigma_k + \sum_{j\neq l} g_{lj}(k)   \p_j(k) } \right)
 \\
 &  = \frac{ 1}{N} \cdot  \W(\bs,\bp),
\end{aligned}
\end{equation}
where $\W(\bs,\bp)$ is the social welfare defined in \eqref{eq:yyy:sw}.
This implies that the individual objective of each user is aligned with the social objective.
Hence, the socially efficient outcome $(\bs^\circ,\bp^\circ ) $ that maximizes the social welfare $\W(\bs,\bp)$ is also an equilibrium of the Taxation Version of the Channel Selection Game $\C$. Formally,

\begin{lemma}\label{lemma:mcwa:tax}
For the Channel Selection Game $\C$,
we can achieve at least one efficient NE, i.e., $(\bs^\circ,\bp^\circ ) $, by implementing the Taxation Mechanism with the following taxing rule:
$$
\r_i = \frac{N-1}{N},\ \ex_i = 0,\quad \forall i\in\N.
$$
At this equilibrium $(\bs^\circ,\bp^\circ ) $, all users share the (maximum) social welfare equally (i.e., Max-min fairness).
\end{lemma}
\begin{proof}
This lemma can be proved by Theorem \ref{thm:efficiency} and Lemma \ref{lemma:fair1} directly.
\end{proof}

Next we show how to interpret the tax, how to impose the tax, and how to redistribute the tax in this MCWA model.
Note that in the MCS model, we can view the taxation process as the transfer of money among users, due to the monetization of the user payoff.
In the MCWA model, however, the taxation process cannot be viewed as the money transfer, as the user payoff (i.e., channel capacity) is not monetized.

In this MCWA model, based on the definition of user payoff in \eqref{eq:yyy:payoff}, we can interpret the tax imposed on a user as ``\emph{a portion of channel capacity that the user achieves}''.
Hence, to impose a certain tax on a user, we essentially ask the user to contribute a certain capacity for transmitting other users' data.
To redistribute the tax of a user to other users, we essentially assign the capacity contributed by a user to other users.
Obviously, to achieve the above cooperative data transmission, mobile users need to stay close enough so that they can connect with each other locally via device-to-device technologies such as Wi-Fi and Bluetooth.



==> app-proof-lemma1.tex <==


%\subsection{Proof for Lemma \ref{lemma:1}}\label{app:0}

\begin{proof}
It is easy to see that with a flat tax rate, say $ \r $, the social welfare of $\G(\bex, \br)$ is
$ \Wx (\bs) = \sum_{i\in\N} \ux_i(\bs) = (1 - \r + \r \bg) \cdot \W (\bs) $, where $\W (\bs)$ is social welfare of $\G$. Hence, an SE of $\G(\bex, \br)$ must be an SE of $\G$, and vice versa.
\end{proof}

==> app-proof-lemma2.tex <==

%\subsection{Proof for Lemma \ref{lemma:fair1}}\label{app:2}

\begin{proof}
By \eqref{eq:payoff-exemption},
each player's payoff under the efficient equilibrium $\bs^*$ achieved from the flat tax rates \eqref{eq:flat-rate} is:
$$
\ux_i(\bs^*) =  \frac{ \overline{\W}  }{N} -  \frac{  \Delta}{N}  + \ex_i,
$$
where  $\Delta = \sum_{i \in \N}\ex_i $ is the sum of all players' tax exemptions.

Therefore, if $  \ex_i =  \ex_j = \omega,  \forall i,j\in\N$, then we have:
$$
\ux_i(\bs^*) =   \frac{ \overline{\W}  }{N} , \quad \forall i \in \N.
$$

Next we show that the above solution is equivalent to a Max-min solution with the \emph{transferrable utility}, which is given by the following optimization problem \cite{max-min}:
\begin{equation}
\begin{aligned}
 \max_{\bs} & \ \min_{i \in \N} \
\left( \u_i(\bs) + v_i  \right)
\\
s.t. &  \sum_{i\in \N} v_i = 0 ,
\end{aligned}
\end{equation}
where $  v_1, \cdots, v_N $ denote the internal utility transfer among players, and $\u_i(\bs) + v_i$ denotes the actual payoff of each player $i \in \N$ after utility transferring.
The constraint implies that the internal utility transfer among players must be balanced.

%That is, all players share the total social welfare equally, which is a special case of the Max-min fairness \cite{max-min}.
Solving the above optimization problem, we can obtain the following Max-min solution: $\bs^\dag = \bs^\circ$ and
$$
\ v_i^\dag = \frac{ \overline{\W}  }{N} - \u_i(\bs^\circ), \ \forall i\in \N.
$$
It is easy to see that under the above Max-min solution, the achieved payoff of each player $i$  is
$$
\u_i(\bs^\dag) + v_i^\dag = \frac{ \overline{\W}  }{N} ,
$$
which is equivalent to that in Lemma \ref{lemma:fair1}.
\end{proof}



==> app-proof-lemma3.tex <==

%\subsection{Proof for Lemma \ref{lemma:fair2}}\label{app:3}

\begin{proof}
By \eqref{eq:payoff-exemption},
each player's payoff under the efficient equilibrium $\bs^*$ achieved from the flat tax rates \eqref{eq:flat-rate} is:
$$
\ux_i(\bs^*) =  \frac{ \overline{\W}  }{N} -  \frac{  \Delta}{N}  + \ex_i,
$$
where  $\Delta = \sum_{i \in \N}\ex_i $ is the sum of all players' tax exemptions.

Therefore, if $  \ex_i =  d_i + \omega , \forall i \in \N$, then we have:
$$
\textstyle
\ux_i(\bs^*) = \frac{ \overline{\W}  }{N} - \frac{\sum_j d_j }{N} + d_i
,\quad \forall i\in\N.
$$

Next we show that the above solution is equivalent to a Nash bargaining solution with the  \emph{transferrable utility}, which is given by the following optimization problem \cite{Nash-bargaining}:
\begin{equation}
\begin{aligned}
\bs^\dag = \arg \max_{\bs} & \ \prod_{i \in \N}
\left( \u_i(\bs) + v_i - d_i \right)
\\
s.t. &  \mbox{ (a) } \sum_{i\in \N} v_i = 0 ,
\\
&  \mbox{ (b) } \u_i(\bs) + v_i \geq d_i, \ \forall i\in\N,
\end{aligned}
\end{equation}
where $  v_1, \cdots, v_N $ denote the internal utility transfer among players, $\u_i(\bs) + v_i$ denotes the actual payoff of each player $i \in \N$ after utility transferring, and $d_i$ denotes the disagreement point of each player $i \in \N$.
The first constraint implies that the internal utility transfer among players must be balanced.
The second constraint implies that each player achieves a payoff higher than his disagreement point.

Solving the above optimization problem, we can obtain the following Nash bargaining solution: $\bs^\dag = \bs^\circ$ and
$$
\ v_i^\dag = \frac{ \overline{\W}  }{N} - \frac{\sum_j d_j }{N} + d_i - \u_i(\bs^\circ), \ \forall i\in \N.
$$
It is easy to see that under the above Nash bargaining solution, the achieved payoff of each player $i$  is
$$
\u_i(\bs^\dag) + v_i^\dag = \frac{ \overline{\W}  }{N} - \frac{\sum_j d_j }{N} + d_i,
$$
which is equivalent to that in Lemma \ref{lemma:fair2}.
\end{proof}


==> app-proof-lemma4.tex <==
%\subsection{Proof for Lemma \ref{lemma:fair3}}\label{app:4}

\begin{proof}
By \eqref{eq:payoff-exemption},
each player's payoff under the efficient equilibrium $\bs^*$ achieved from the flat tax rates \eqref{eq:flat-rate} is:
$$
\ux_i(\bs^*) =  \frac{ \overline{\W}  }{N} -  \frac{  \Delta}{N}  + \ex_i,
$$
where  $\Delta = \sum_{i \in \N}\ex_i $ is the sum of all players' tax exemptions.

Let $\phi_i$ denote the payoff of each player $i \in \N $ in the Shapley value \cite{Shapley-value}. Then, $\sum_{i\in\N} \phi_i = \overline{\W} $ according to  \cite{Shapley-value}. Namely, in the Shapley value, the social welfare is maximized and fully distributed to all players.
Therefore, if $  \ex_i =  \phi_i + \omega , \forall i \in \N$, then we have: $\Delta = \overline{\W} + N \omega $ and
$$
\textstyle
\ux_i(\bs^*) = \phi_i
,\quad \forall i\in\N,
$$
which is equivalent to that in the Shapley value \cite{Shapley-value}.
\end{proof}


==> app-proof-mcs0.tex <==
\begin{proof}
On one hand, if one of the conditions in \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3} is not satisfied, then the strategy $\bs_i $ is not feasible as explained early. Thus,  if $\bs_i $ is feasible, then the conditions \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3} must be satisfied.
One the other hand, if the conditions \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3} are satisfied, then the strategy $\bs_i $ can be implemented by user $i$ successfully, hence is feasible.
\end{proof}


==> app-proof-mcs1.tex <==

%\subsection{Proof for Lemma \ref{lemma:mcs:potential}}\label{app:5}


\begin{proof}
To prove that the Task Selection Game $\T$ is a potential game with the potential function  $\Phi(\bs)$ given in \eqref{eq:xxx:pf}, we   need to show that for every user $i\in \N$ and any  strategies $\bs_i,\bs_i' \subseteq \S_i $ of user $i$, the following equation holds:
\begin{equation}\label{eq:pf-proof}
 \u_i (\bs_i, \bs_{-i} ) - \u_i (\bs_i', \bs_{-i} )
=
\Phi (\bs_i, \bs_{-i} ) - \Phi (\bs_i', \bs_{-i} ),
\end{equation}
under any feasible strategy profile $\bs_{-i}$ of other users.

We first show that equation \eqref{eq:pf-proof} holds when user  $i$ only changes the execution order,
while not changing the task selection. Namely, $\bs_i $ and $\bs_i' $ contain the same task set (but different execution orders).
It is easy to see that
$$
M_k (\bs_i, \bs_{-i}) = M_k (\bs_i', \bs_{-i}), \quad \forall k\in\S,
$$
that is, the number of users executing each task $k \in \S$ does not change  when user $i$ only changes the execution order. This implies that the achieved reward and the incurred execution cost of user $i$ will not change.
Thus, by \eqref{eq:xxx:payoff}, we have:
\begin{equation*}
\begin{aligned}
& \u_i (\bs_i, \bs_{-i} ) - \u_i (\bs_i', \bs_{-i} ) =
c_i^{\textsc{tr}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i'),
\end{aligned}
\end{equation*}
where only the travelling cost of user $i$ is changed.
For the potential function  in \eqref{eq:xxx:pf}, we also have:
\begin{equation*}
\begin{aligned}
\Phi (\bs_i, \bs_{-i} ) - \Phi (\bs_i', \bs_{-i} ) =
c_i^{\textsc{tr}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i').
\end{aligned}
\end{equation*}
This is because the change of user $i$'s execution order does not affect the execution costs and travelling costs of other users. Based on the above, we can see that equation \eqref{eq:pf-proof} holds when user $i$ changes the execution order only.


We then show that equation \eqref{eq:pf-proof} holds when player $i$ changes his strategy from $\bs_i $ to $\bs_i' $ by removing a task $\tau \in \bs_i$, i.e., $\bs_i' = \bs_i / \{ \tau \}$.
According to \eqref{eq:xxx:payoff}, we have:
\begin{equation*}
\begin{aligned}
& \u_i (\bs_i, \bs_{-i} ) - \u_i (\bs_i', \bs_{-i} )
\\
= &  \sum_{k \in \bs_i }  \frac{V_k}{M_k (\bs_i , \bs_{-i})}
 -
c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i)
\\
&
-
\sum_{k \in \bs_i'}  \frac{V_k}{M_k (\bs_i', \bs_{-i})}
+
c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i')
\\
= & \ \frac{V_\tau}{M_\tau (\bs_i , \bs_{-i})}  +
c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i') -
c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i) .
\end{aligned}
\end{equation*}
For the potential function  in \eqref{eq:xxx:pf}, we have:
\begin{equation*}
\begin{aligned}
& \Phi (\bs_i, \bs_{-i} ) - \Phi (\bs_i', \bs_{-i} )
\\
= &  \sum_{k \in \S}   \sum_{m=1}^{M_k(\bs_i, \bs_{-i})} \frac{V_k}{m}
 - \sum_{j\in\N} c_j^{\textsc{ex}} (\bs_j)
 - \sum_{j\in\N} c_j^{\textsc{tr}} (\bs_j)
 \\
 & - \sum_{k \in \S} \!\!\!\!  \sum_{m=1}^{M_k(\bs_i', \bs_{-i})} \frac{V_k}{m}
+ \sum_{j\neq i} c_j^{\textsc{ex}} (\bs_j)
 + \sum_{j\neq i} c_j^{\textsc{tr}} (\bs_j) + c_i^{\textsc{ex}} (\bs_i')+ c_i^{\textsc{tr}} (\bs_i')
 \\
 = &  \!\!\!\!  \sum_{m=1}^{M_\tau(\bs_i, \bs_{-i})}  \frac{V_\tau}{m}  -  \!\!\!\!  \sum_{m=1}^{M_\tau(\bs_i', \bs_{-i})} \frac{w_\tau}{m}
  +
c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i') -
c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i)
 \\
 = & \ \frac{V_\tau}{M_\tau (\bs_i , \bs_{-i})}  +
c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i') -
c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i) .
\end{aligned}
\end{equation*}
The last equation is due to  $ M_\tau(\bs_i , \bs_{-i}) = M_\tau(\bs_i', \bs_{-i}) + 1$ and $ M_k(\bs_i , \bs_{-i}) = M_k(\bs_i', \bs_{-i}) $ for all $k \neq \tau$.
Based on the above, we can see that   equation \eqref{eq:pf-proof} holds when user $i$ removes a task from his strategy.
Similarly, we can show that  equation \eqref{eq:pf-proof} holds when user $i$ adds a task into his strategy.

Using the above results iteratively, we can show that
  equation \eqref{eq:pf-proof} holds when user $i$ changes his strategy from an arbitrary $\bs_i $ to an arbitrary $\bs_i' $.
\end{proof}


==> app-proof-mcs2.tex <==
%\subsection{Proof for Lemma \ref{lemma:mcs:NE}}\label{app:6}

\begin{proof}
We will show that the outcome $\bs^*$ given by \eqref{eq:xxx:NE} is an NE of  $\T$.
According to \eqref{eq:xxx:NE}, we find that for any $i \in \N$,
$$
\Phi(\bs_i^*, \bs_{-i}^*) \geq \Phi(\bs_i ', \bs_{-i}^*), \quad \forall \bs_i ' \subseteq \S_i.
$$
By Lemma \ref{lemma:mcs:potential}, we further have: for any   $i\in \N$ and $\bs_i ' \subseteq \S_i$,
$$
 \u_i (\bs_i^*, \bs_{-i}^* ) - \u_i (\bs_i', \bs_{-i}^* )
=
\Phi (\bs_i^*, \bs_{-i}^* ) - \Phi (\bs_i', \bs_{-i}^* ).
$$
Hence, we have the following observations:
$$
 \u_i (\bs_i^*, \bs_{-i}^* ) \geq \u_i (\bs_i', \bs_{-i}^* ), \quad \forall \bs_i ' \subseteq \S_i, i\in\N,
$$
which implies that the outcome $\bs^*$ in \eqref{eq:xxx:NE} is an NE of  $\T$.
\end{proof}

==> app-proof-mcs3.tex <==

%\subsection{Proof for Lemma \ref{lemma:mcs:tax}}\label{app:7}


\begin{proof}
This lemma can be proved by Theorem \ref{thm:efficiency} and Lemma \ref{lemma:fair1} directly.
\end{proof}

==> app-proof-theorem1.tex <==

%\subsection{Proof for Theorem \ref{thm:efficiency}}\label{app:0x}


\begin{proof}
With the flat tax rate $\r = \frac{N-1}{N-1+\bg}$, we can compute the payoff of each player $i$ in the Taxation Version $\G (\bex, \br) $ as follows:
$$
\ux_i(\bs) = c \cdot \sum_{j\in\N} \u_j(\bs) - c\cdot \Delta + \ex_i
$$
$$
~~~~~ = c \cdot \W(\bs)  - c\cdot \Delta + \ex_i .
$$
%where $a_i = \frac{\bg}{N-1+\bg}  $ and $b_i =  \ex_i-\sum_{j\in \N } \frac{\ex_j \bg}{N-1+\bg} $ are constants (with respect to $\bs$).
Moreover, the social welfare in $\G (\bex, \br) $ can be computed by:
$$
\Wx (\bs) = \sum_{i\in\N} \ux_i(\bs) = c\cdot N \cdot \W (\bs) + \Delta \cdot (1-c \cdot N).
$$
This implies that an SE of $\G (\bex, \br) $ (which is also an SE of $\G$ by Lemma \ref{lemma:1})
must be an equilibrium of $\G (\bex, \br) $.
Namely, $\G (\bex, \br) $  has at least one efficient outcome (i.e., the above SE)
that maximizes the social welfare of $\G (\bex, \br) $ and $\G$.
\end{proof}

==> app-proof-theorem2.tex <==

%\subsection{Proof for Theorem \ref{thrm:unique}}\label{app:1}

\begin{proof}
We have shown the sufficiency of \eqref{eq:flat-rate} in Theorem \ref{thm:efficiency}, and only need to prove the necessity of \eqref{eq:flat-rate}.
Hence, in the following, we will prove ``a taxing rule $\{\bex, \br\}$ is efficient for all static strategic games (with common knowledge), only if the tax rates satisfy \eqref{eq:flat-rate}'', or equivalently, ``there does \emph{not} exist a taxing rule $\{\bex, \br\}$ without satisfying \eqref{eq:flat-rate} that is efficient for \emph{all} static strategic games (with common knowledge)''. 

%To show this, we consider a static strategic game with the following strictly concave payoff functions:
%$$
%\u_i (\bs) = a_i \cdot f_i (\bs), \quad \forall i\in \N,
%$$
%where $a_i > 0 $ is a system parameter and $f_i (\bs)$ is a strictly concave function.
%Obviously, the social welfare
%$$
%\W(\bs) = \sum_{i\in\N} a_i \cdot f_i (\bs)
%$$
%is also a strictly concave function, and thus has a unique SE outcome $ \bs^\circ $ given by the following conditions:
%$$
%\frac{\partial \W(\bs) }{ \partial \s_i } =   \sum_{i\in\N} a_i \cdot \frac{\partial f_i (\bs)}{ \partial \s_i } = 0,\quad \forall i\in\N.
%$$
%
%Under a taxing rule $\{\bex, \br\}$, we can obtain the new payoff of each player according to \eqref{eq:payoff-tax}, i.e.,
%$$
%\ux_i (\bs)   = \u_i (\bs) - ( \u_i (\bs) - \ex_i ) \cdot \r_i
%  + \sum_{j \neq i}  \frac{( \u_j (\bs) - \ex_j ) \cdot \r_j \cdot \bg }{N-1}.
% $$
%Thus, the NE outcomes $\bs^*$ of the new game are give by the following conditions:
%$$
%a_i (1-\r_i) \cdot \frac{\partial f_i (\bs)}{ \partial \s_i} +
%\sum_{j\neq i} \frac{a_j \r_j \bg}{N-1} \cdot \frac{\partial f_j (\bs)}{ \partial \s_i } = 0,\quad \forall i\in\N.
%$$
%
%To guarantee the equivalence of the above NE conditions and SE conditions under \emph{all possible} system parameters $\{a_i, i \in \N\}$, we need such a taxing rule $\{\bex, \br\}$ with which each coefficient in the NE conditions is proportional to the corresponding coefficient in the SE conditions. That is,
%$$
%\frac{a_i (1-\r_i) }{a_i} = \frac{a_j \r_j \bg }{ a_j (N-1)}, \quad \forall j\neq i, \quad \forall i\in\N.
%$$
%It is easy to see that the only taxing rates that satisfy the above conditions are:
%$$
%\r_i = \frac{N-1}{N-1+\bg} , \forall i\in\N
%$$
%given in \eqref{eq:flat-rate}.

To prove this, we only need to find a static strategic game in which the taxing rule $\{\bex, \br\}$ satisfying \eqref{eq:flat-rate} is the \emph{only} taxing rule that can generate efficient outcomes.
Let us consider such a static strategy game with the following payoff functions:
$$
\u_i(\bs) = a_i \cdot \s_i -  \frac{(\s_1 + \cdots + \s_N)^2}{N}, \quad \forall i\in \N ,
$$
where $a_i \neq a_j$ for all $i,j\in\N$.
Intuitively, it models a simple game situation where players consume a limited resource (e.g., wireless frequency band).
The first term in the payoff denotes the benefit of each player for consuming resource.
The second term in the payoff denotes the cost of each player due to the congestion of different players, which increases convexly with the total consumption of all players.

It is easy to see that in the above game, the social welfare
$$
\W(\bs) = \sum_{i\in\N} a_i \cdot \s_i - (\s_1 + \cdots + \s_N)^2
$$
 is a strictly concave function, and thus has a unique SE:
\begin{equation}\label{eq:sko}
\s_{i'}^\circ =  \frac{a_{i'}}{2},\  \s_j^\circ = 0 , \quad \forall j\neq {i'} ,
\end{equation}
where $ {i'} $ is the player with the maximum consuming factor $a$, i.e., $a_{i'} > a_j$ for all $j \neq {i'}$.
It is important to note that \eqref{eq:sko} is the unique SE of the above game.
This implies that if a taxing rule $\{\bex, \br\}$ is efficient, it must generate an equilibrium outcome equivalent to the unique SE in \eqref{eq:sko}.
%In other words, the unique SE in \eqref{eq:sko} must be an NE of the Taxation Version of the above game (with an efficient taxing rule).


Now we consider the Taxation Version of the above game with the taxing rule $\{\bex, \br\}$.
By \eqref{eq:payoff-tax},
the new payoff of each player $i\in \N$ in the Taxation Version with $\{\bex, \br\}$ is
$$
\ux_i (\bs)   = \u_i (\bs) - ( \u_i (\bs) - \ex_i ) \cdot \r_i
  +   \sum_{j\neq i} \frac{( \u_{j} (\bs) - \ex_{j} ) \cdot \r_{j} \cdot \bg }{N-1} ,
 $$
which is strictly concave with respect to $\s_i$.
Thus, given the choices $\bs_{-i}$ of other players, the best response of player $i$ is given by the following first-order condition:
\begin{equation}\label{eq:first-order}
 \begin{aligned}
\frac{\partial \ux_i  (\bs )}{ \partial \s_i }=  &
\left(a_i -  \frac{2 (\s_1 + \cdots + \s_N)}{N} \right) \cdot (1 - \r_i)
 \\
& - \sum_{j\neq i} \frac{2 (\s_1 + \cdots + \s_N)}{N} \cdot\frac{ \r_j  \cdot \bg }{N-1} = 0.
\end{aligned}
\end{equation}



Suppose $a_i$ is the maximum consuming factor of all player, i.e., $a_i> a_j,\forall j\neq i$.
According to  \eqref{eq:sko}, the unique SE (of the original game) is
$
\s_i^\circ =  \frac{a_i}{2}$ and $\s_j^\circ = 0, \forall j \neq i
$.
Based on the above discussion, if the taxing rule $\{\bex, \br\}$ is efficient, it must generate an equilibrium outcome equivalent to the above SE. In other words, the above SE must be an NE of the Taxation Version with $\{\bex, \br\}$.
This implies that $\s_i^\circ =  \frac{a_i}{2}$ is the best response of player $i$ given the choices $\bs_{-i}^\circ  = \boldsymbol{0}$ of other players, that is, it satisfies the first-order condition~in~\eqref{eq:first-order}:~~~~~~~~
\begin{equation}
 \begin{aligned}
\frac{\partial \ux_i(\s_i^\circ, \bs_{-i}^\circ )} { \partial \s_i }
& = \left(a_i - \frac{a_i}{N} \right)(1-\r_i) - \frac{a_i}{N} \sum_{j\neq i} \frac{ \r_j    \bg }{N-1}
\\
& = \frac{a_i}{N} \cdot \left( (N-1)(1-\r_i) -  \sum_{j\neq i} \frac{ \r_j  \bg }{N-1}  \right)
\\
& = 0.
\end{aligned}
\end{equation}
Associating the above  conditions for all $i\in\N$, we have the following necessary conditions for an efficient taxing rule (for the above static strategic game):
\begin{equation}\label{eq:funcset}
\left\{
 \begin{aligned}
(N-1)(1-\r_1) -  \sum_{j\neq 1} \frac{ \r_j  \bg }{N-1} = 0
\\
...
\\
(N-1)(1-\r_N) -  \sum_{j\neq N} \frac{ \r_j  \bg }{N-1} = 0
\end{aligned}
\right.
\end{equation}
By summing up all equations listed above, we have:
$$
(N-1)N  - (N-1) \sum_{i\in \N} \r_i - \bg \sum_{i\in \N} \r_i = 0,
$$
and hence,
$$
\sum_{i\in \N} \r_i = \frac{(N-1)N}{N-1+\bg}.
$$
Substitute the above formula into \eqref{eq:funcset}, we can obtain:
\begin{equation}
\r_i = \frac{N-1}{N-1+\bg}, \quad \forall i\in \N,
\end{equation}
which are exactly the tax rates given in \eqref{eq:flat-rate}.



%Thus, the NE outcomes $\bs^* $ of the new game are give by the following first-order conditions:
%\begin{equation}
%\left\{
% \begin{aligned}
%\frac{\partial \ux_1 (\s_1^*, \s_2^* )}{ \partial \s_1 } & =
%(a_1 - \s_1^* - \s_2^* ) \cdot (1 - \r_1) - (\s_1^* + \s_2^*) \cdot \r_2  \cdot \bg  \\
%& = 0,
%\\
%\frac{\partial \ux_2 (\s_1^*, \s_2^* )}{ \partial \s_2 } & =
%(a_2 - \s_1^* - \s_2^* ) \cdot (1 - \r_2) - (\s_1^* + \s_2^*) \cdot \r_1  \cdot \bg  \\
%& = 0.
%\end{aligned}
%\right.
%\end{equation}

From the above discussion, we show that in the above static strategic game, the tax rates given in \eqref{eq:flat-rate} is necessary for an efficient taxing rule.
This implies that if a taxing rule $\{\bex, \br\}$ is efficient for \emph{all} static strategic games (with common knowledge), then the tax rates must satisfy \eqref{eq:flat-rate}.
\end{proof}


==> section-app.tex <==
\newpage


Online technical report for ``\textbf{\emph{Achieving Efficient and Fair Equilibrium Through Taxation}}'' submitted to  {ACM SIGMETRICS 2017}.
Outline of the report:

{\it
\begin{itemize}
  \item \ref{app:0}: Proof for Lemma \ref{lemma:1}
  \item \ref{app:0x}: Proof for Theorem \ref{thm:efficiency}
  \item \ref{app:1}: Proof for Theorem \ref{thrm:unique}
  \item \ref{app:2}: Proof for Lemma \ref{lemma:fair1}
  \item \ref{app:3}: Proof for Lemma \ref{lemma:fair2}
  \item \ref{app:4}: Proof for Lemma \ref{lemma:fair3}
  \item \ref{app:5a}: Proof for Lemma \ref{lemma:mcs-feasibility}
  \item \ref{app:5}: Proof for Lemma \ref{lemma:mcs:potential}
  \item \ref{app:6}: Proof for Lemma \ref{lemma:mcs:NE}
  \item \ref{app:7}: Proof for Lemma \ref{lemma:mcs:tax}
  \item \ref{app:8}: Simulations for Application I -- MCS
  \item \ref{app:9}: Analysis for Application II -- MCWA
\end{itemize}
}

\appendix

\section{Appendix}


\subsection{Proof for Lemma \ref{lemma:1}}\label{app:0}

\input{app-proof-lemma1}


\subsection{Proof for Theorem \ref{thm:efficiency}}\label{app:0x}

\input{app-proof-theorem1}


\subsection{Proof for Theorem \ref{thrm:unique}}\label{app:1}

\input{app-proof-theorem2}


\subsection{Proof for Lemma \ref{lemma:fair1}}\label{app:2}

\input{app-proof-lemma2}



\subsection{Proof for Lemma \ref{lemma:fair2}}\label{app:3}

\input{app-proof-lemma3}


\subsection{Proof for Lemma \ref{lemma:fair3}}\label{app:4}

\input{app-proof-lemma4}


\subsection{Proof for Lemma \ref{lemma:mcs-feasibility}}\label{app:5a}

\input{app-proof-mcs0}



\subsection{Proof for Lemma \ref{lemma:mcs:potential}}\label{app:5}

\input{app-proof-mcs1}

\begin{figure*}
\hspace{-6mm}
	\centering
\includegraphics[width=2.3in]{Figures/MCS-simu-sw1}
--
\includegraphics[width=2.3in]{Figures/MCS-simu-sw2}
--
\includegraphics[width=2.3in]{Figures/MCS-simu-sw3}
	\caption{Social Welfare under SE and NE: (a) Walking Users; (b) Bike Users; (c) Driving Users.}
\label{fig:mcs-simu-sw}
\end{figure*}


\subsection{Proof for Lemma \ref{lemma:mcs:NE}}\label{app:6}

\input{app-proof-mcs2}




\subsection{Proof for Lemma \ref{lemma:mcs:tax}}\label{app:7}

\input{app-proof-mcs3}



\subsection{Simulations for Application I -- MCS}\label{app:8}

\input{app-mcs-simu}



\subsection{Analysis for Application II -- MCWA}\label{app:9}

\input{app-mcwa}



==> section4-app-MCS.tex <==


\subsection{Application I: Mobile Crowd Sensing}

%Due to space limit, we leave the discussion regarding MCS in our online Technical report \cite{report}.

With the development and proliferation of   smartphones with rich build-in sensors and advanced computing capabilities,
we are witnessing  a new sensing paradigm of \emph{Mobile Crowd Sensing (MCS)} \cite{xxx-2,xxx-3,xxx-4,xxx-5,xxx-6}, which relies  on the active participation and contributions of  mobile users by using their smartphones.
Comparing with the traditional approach of deploying  sensor networks, MCS has the advantages of low deploying cost, high sensing coverage, and high flexibility.
Hence, it has found  a wide range of applications in environment, infrastructure, and community monitoring \cite{mcs-app1,mcs-app2,mcs-app3,mcs-app4}.

In this application, we consider a general MCS model motivated by  those in \cite{xxx-4,xxx-5,xxx-6}, where a sensing platform announces the sensing tasks and   mobile users simultaneously choose  the sensing tasks to execute.
The task selections of different users are dependent, leading to a static strategic game, called \emph{Task Selection Game}.
We will show how to implement
the Taxation Mechanism in the Task Selection Game, and how it will steer the game equilibrium outcome to a desirable one.

\subsubsection{System Model}
We consider an MCS system with a sensing platform and a set $\N = \{1,\cdots,N\}$ of mobile smartphone users.
The platform announce a set $\S = \{1,\cdots,S\}$ of sensing tasks.
Each task can represent a specific sensing event at a particular time and  location, or a set of periodic sensing events within a certain time period, or a set of sensing events at multiple locations.
Each task $k \in \S$ is associated with a \emph{reward} $V_k$, denoting the money to be paid to the users who executes the task successfully.
When multiple users execute the same task, they will share the reward \emph{equally}   as in \cite{xxx-4}.
This makes the task selections of different users coupled with each other, leading to a   strategic game.

%\subsubsection*{Task Model}

\emph{\textsf{Task Model:}}
We consider a general task model, where tasks are (i)  \emph{location-dependent}: each task $k \in \S$ is associated with a target location $L_k $ at which the task will be executed;\footnote{Examples of such tasks includes the measurement of   traffic speed  at a particular road conjunction or the air quality of a particular location.
Note that our analysis can be easily extended to the tasks with multiple target locations, by simply dividing each task into multiple sub-tasks, each associated with one target location.}
and (ii) \emph{time-sensitive}: each task $k \in \S$ is associated with a valid time period $T_k \eq [T_k^{\dag},\ T_k^{\ddag}]$ within which the task must be executed.
\revvm{Such a task model differs from those in \cite{xxx-4,xxx-5,xxx-6} in the following aspects.
First, \cite{xxx-5,xxx-6} considered the location-dependent tasks without the time-sensitivity constraint, where each task can be executed at any time.
Second, \cite{xxx-4} considered the location-dependent tasks with the strict time-sensitivity constraint, where each task must be executed at a particular time.
In our model, each task can be executed within a given valid time period.
When choosing a very large valid time period, our task model degenerates to those in \cite{xxx-5,xxx-6};
when choosing a very small valid time period, our task model degenerates to that in \cite{xxx-4}.
Hence, our task model generalizes those in \cite{xxx-5,xxx-6,xxx-4}, which can be viewed as two special (extreme) cases of our model.}

% Later we will show that such a model extension is not trivial, as it introduces

%\subsubsection*{User Model}

\emph{\textsf{User Model:}}
Each user $i \in \N $ can choose one or multiple tasks (to execute) from a set of tasks $\S_i \subseteq \S$ available to him.
The availability of a task to a user depends on factors such as the user's device capability, time availability, mobility, and experience.
When executing a task successfully, the user can get the task reward solely or share the task reward equally with other users who also execute the task.
The \emph{payoff} of each user is defined as the difference between the achieved \emph{reward} and the incurred \emph{cost}, mainly including the execution cost and  the travelling cost (to be described below).

When executing a task, a user needs to consume some time and device resource (e.g., energy, bandwidth, and CPU resource), hence incur certain \emph{execution cost}.
Such an execution cost and time depends on both the task natures (e.g., one-shot or periodic sensing) and the user characteristics  (e.g., experienced or inexperienced, resource limited or adequate).
Let $T_{i, k}$ and $C_{i, k}$ denote the time and cost of user $i \in \N $ for executing task $ k \in \S_i $.
Each user $i$ has a total budget $C_i$ of resource that can be used for executing tasks.

\begin{figure}
	\centering
\includegraphics[width=3.5in]{Figures/MCS-model-new}
	\caption{An Example of Location-Dependent Time-Sensitive MCS Model. Each route denotes the task selection and task execution order for each user.}
\label{fig:mcs-model}
\end{figure}

Moreover, in order to execute a task, a user needs to move to the target location of the task (in a certain travelling speed), which may incur certain \emph{travelling cost}.
After executing a task, the user will stay at that location (to save travelling cost) until he moves to a new location to execute a new task.
With a litter abuse of notation, we denote $L_i $ as the initial location of user $i\in \N$.
The travelling cost and speed mainly depend on the type of transportation that the user takes.
For example, a walking user has a low  speed and cost, while a driving user may have a high speed and cost.
Let  $\widetilde{C}_i$ and $R_i$    denote the travelling  cost (per unit of distance) and speed (m/s) of user $i\in \N$.

Figure \ref{fig:mcs-model} illustrates an example of such a location-dependent time-sensitive MCS model with $N=3$ users and $S=9$ tasks, where each triangle denotes a task (and its target location) and each circle denotes a user (and his initial location).
%The table in the upper-left corner lists the reward and valid time period  of each task.
Each dashed route initiating from a user denotes the user's moving trajectory, indicating the set of tasks that the user chooses and the order of tasks to be executed.
In this example, user $1$ chooses to execute tasks $\{1,2,3,4\}$ in order, user $2$ chooses to execute tasks $\{3,5,6\}$ in order, and user 3 chooses to execute tasks $\{7,8,9\}$ in order.
Note that task $3$ is executed by users $1$  and $2$, hence its reward $3.0$ is shared by these two users  equally.
Thus, the total reward of user $1$ is $1+1.3+ \frac{3.0}{2} + 0.8 = 4.6$,
the total reward of user $2$ is $\frac{3.0}{2} + 1.5+2.8 = 5.8$, and the total reward of user $3$ is $1+1.8+2 = 4.8$.


%\comm{In our model, is it possible for multiple users to execute the same task? If so, how would be the reward be splitted among multiple users? }


\emph{\textsf{Our Studied Problem:}}
 Due to the existence of travelling cost (and the valid time of tasks), we need to consider not only the \emph{task selection} (i.e., the set of tasks to be executed) but also the \emph{execution order} of the selected tasks for each user.
As illustrated in Figure \ref{fig:mcs-model}, such a task execution order is very important, as it affects not only the user's travelling cost but also whether the tasks can be executed successfully within their valid time periods.
For example, if user $1$ chooses to execute task $4$ first (within the time period [14:00, 18:00]), he cannot execute tasks $\{1,2,3\}$ within their valid time periods (all of which are earlier than 13:00).

This is also the key difference between our problem and that in \cite{xxx-4}, which only focused on  the task selection, without considering the task execution order.\footnote{In \cite{xxx-4}, each task is associated with a specific execution time, hence the execution order is inherently given as long as the tasks are selected.}
Note that introducing the task execution order into the user strategy  will greatly complicate the problem, as even given the task selection, the task   order optimization is still an NP-hard problem.
Thus, our problem (joint task selection and order optimization) is much more challenging than that (task selection only) in \cite{xxx-4}.

%Figure \ref{fig:mcs-model} illustrates an example of task selection and executing order in an MCS model with $N=3$ users and $S=9$ tasks, where the route initiating from each user denotes the set of tasks that the user selects and the order of tasks to be executed.


%Intuitively, to save the travelling cost, a user may choose to execute the tasks near to him first, and then the tasks far from him; while to meet the tasks' time-sensitivity constraints, a user need to execute the the tasks close to deadline first, and then the tasks with a long valid time.

% \input{section4-app-MCS-edge}

\subsubsection{Game Formulation}

 As mentioned above, the strategy of each user $i\in \N$ is to choose a set of available tasks (to execute) and the execution order of the selected tasks, aiming at maximizing his payoff.
Such a strategy of user $i$ can be formally characterized  by an \emph{ordered} task set $\bs_i \eq \{ k_i^1, \cdots, k_i^{|\bs_i|} \} \subseteq \S_i $, where the $j$-th element $k_i^j $ denotes the $j$-th task executed by user $i$.

\emph{\textsf{Strategy Feasibility:}}
A strategy $\bs_i = \{ k_i^1, \cdots, k_i^{|\bs_i|} \}  $ of user $i$ is feasible, only if the time-sensitivity constraints of all selected tasks in $\bs_i$ can be satisfied,
or equivalently, there exists a reasonable execution time vector such that all selected tasks in $\bs_i$ can be executed within their valid time periods.
Let $[T_i^1,\cdots,T_i^{|\bs_i|}]$ denote an execution time vector of user $i$, where $T_i^j$ denotes the execution time for the $j$-th task $k_{i}^j$.
Then, $[T_i^1,\cdots,T_i^{|\bs_i|}]$ is feasible, only if (i) it satisfies the time-sensitivity constraints of all selected tasks, i.e.,
\begin{equation}\label{eq:mcs-fs1}
T_{k_i^j}^{\dag} \leq  T_i^j  \leq  T_{k_i^j}^{\ddag}, \quad j=1,\cdots, |\bs_i|,
\end{equation}
and meanwhile (ii) it is
reasonable in the temporal logic, i.e.,
\begin{equation}\label{eq:mcs-fs2}
\left\{
\begin{aligned}
T_i^{1} & \textstyle
 \geq \frac{D({i} ,  {k_i^{1}})}{r_i},
\\
T_i^{j } &\textstyle \geq T_i^{j-1} + T_{i, k_i^{j-1}} + \frac{D( {k_i^{j-1}}, {k_i^j}) }{r_i}, \  j = 2,\cdots, |\bs_i| ,
\end{aligned}
\right.
\end{equation}
where $D({i} ,  {k_i^{1}}) = |L_{i}- L_{k_i^{1}}| $ denotes the distance between user $i$'s initial location $L_i$ and the first task $k_i^{1}$, $D({k_i^{j-1}}, {k_i^{j}}) = |L_{k_i^{j-1}}- L_{k_i^{j}}| $ denotes the distance between tasks $k_i^{j-1}$ and $k_i^{j}$, and $T_{i, k_i^{j-1}}$ denotes the time for executing task $k_i^{j-1}$.\footnote{The first condition denotes that user $i$ needs to take at least the time $\frac{D({i} ,  {k_i^{1}})}{r_i}$ to reach the first task $k_i^{1}$,
and the following conditions mean that user $i$ needs to takes at least the time $T_{i, k_i^{j-1}} + \frac{D( {k_i^{j-1}}, {k_i^j}) }{r_i}$ to reach task $k_i^{j}$, where the first part of time is used for completing the previous task $k_i^{j-1}$ and the second part of time is used for travelling from task $k_i^{j-1}$ to task $k_i^{j}$.}

Moreover, a strategy   $\bs_i  $ of user $i$  is feasible, only if it satisfies the  resource budget constraint. That is,
\begin{equation}\label{eq:mcs-fs3}
\sum_{k \in \bs_i} C_{i, k} \leq C_i.
\end{equation}

Based on the above, we have the following the feasibility conditions for the user strategy $\bs_i $.

\begin{lemma}[Feasibility]\label{lemma:mcs-feasibility}
A strategy $\bs_i $ of user $i$ is feasible, if and only if the conditions \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3} are satisfied.
\end{lemma}

\input{app-proof-mcs0}

%The strategy of each user $i \in \N $ is to choose a subset $\bs_i \subseteq \S_i $ of available tasks to execute, aiming at maximizing his payoff, considering his maximum budget constraint (i.e., $\sum_{k \in \bs_i} c_{i,k} \leq C_i$).
% The  consist of the strategy profile $\bs = (\bs_1,\cdots,\bs_N)$.

\emph{\textsf{Payoff Definition:}}
Given a feasible strategy profile $\bs \eq (\bs_1,\cdots,\bs_N)$, i.e., the feasible strategies of all users,
we can compute the number of users executing task $k \in \S$, denoted by $M_k (\bs)$, in the following way:
\begin{equation}\label{eq:xxx:mk}
M_k (\bs) = \sum_{i \in \N} \mathbf{1}_{(k \in \bs_i)}, \quad \forall k\in \S,
\end{equation}
where the indicator    $\mathbf{1}_{(k \in \bs_i)} = 1$ if $ k \in \bs_i$, and $  0$ otherwise.
Then, the total reward of each user $i \in \N $ can be computed~by
\begin{equation}\label{eq:xxx:reward}
r_i (\bs) \eq r_i (\bs_i, \bs_{-i}) = \sum_{k \in \bs_i} \frac{V_k}{M_k (\bs)} ,
\end{equation}
which depends on both his own strategy $\bs_i$ and the strategies of other users, i.e., $\bs_{-i} \eq  (\bs_1,\cdots,\bs_{i-1},\bs_{i+1},\cdots,\bs_N) $.
The total execution cost of user $i \in \N $ can be computed by
\begin{equation}\label{eq:xxx:excost}
  c_i^{\textsc{ex}} (\bs_i ) = \sum_{k \in \bs_i} C_{i,k},
\end{equation}
which depends  only on his own strategy  $\bs_i$.
The total travelling cost of user $i \in \N$ can be computed by
\begin{equation}\label{eq:xxx:excost}
  c_i^{\textsc{tr}} (\bs_i ) =     \sum_{j = 1}^{ |\bs_i|  } D({k_i^{j-1}}, {k_i^{j}}) \cdot \widetilde{C}_{i}  ,
\end{equation}
which depends only on his own strategy  $\bs_i$.
Here we denote user $i$ as the $0$-th task $k_i^0$ for the notational convenience.
Based on the above, the payoff of  each user $ i \in \N $ can be written as follows:
\begin{equation}\label{eq:xxx:payoff}
\begin{aligned}
\u_i (\bs) \eq \u_i (\bs_i, \bs_{-i})
  & = r_i (\bs  ) - c_i^{\textsc{ex}} (\bs_i ) - c_i^{\textsc{tr}} (\bs_i )
\\
& = \sum_{k \in \bs_i} \frac{V_k}{M_k (\bs)} - c_i^{\textsc{ex}} (\bs_i ) - c_i^{\textsc{tr}} (\bs_i ).
%& = \sum_{k \in \bs_i} \frac{V_k}{M_k (\bs)} - \sum_{k \in \bs_i} C_{i,k} -    \sum_{j = 1}^{ |\bs_i|  } D({k_i^{j-1}}, {k_i^{j}}) \cdot \widetilde{C}_{i} .
\end{aligned}
\end{equation}


Based on the above discussion, we can formally define the Task Selection Game and the associated NE.
\begin{definition}[\textbf{Task Selection Game}]\label{def:task-game}
The Task Selection Game  $\T \eq (\N, \{\S_i\}_{i\in\N}, \{\u_i\}_{i\in\N})$ is defined by:
\begin{itemize}
  \item  \textbf{Player}: a set $\N = \{1, \cdots , N\}$ of users;
  \item  \textbf{Strategy}: an ordered set of available tasks $\bs_i \subseteq \S_i$ for each user $i\in\N$;
  \item  \textbf{Payoff}: a payoff function   $ \u_i (\bs_i, \bs_{-i})$ defined in \eqref{eq:xxx:payoff} for each user $i\in\N$.
\end{itemize}
\end{definition}


A feasible strategy profile $\bs^* \eq (\bs_1^*,\cdots,\bs_N^*)$ is an NE of the Task Selection Game $\T$, if for every user $i\in\N$,
\begin{equation}\label{eq:xxx:nene}
\begin{aligned}
 \bs_i^* = \arg \max_{\bs_i \subseteq \S_i} \  & \u_i (\bs_i, \bs_{-i}^*) \\
  s.t.\  & \bs_i \mbox{ satisfies \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3}.}
\end{aligned}
\end{equation}
% That is, the strategy $\bs_i^*$ of each user $i$ in $\bs^* $ is his best strategy against the strategy profile $ \bs_{-i}^*$ of other players.
%Hence, no user has the incentive to   unilaterally deviate from  $\bs^* $.
Note that the constraint in \eqref{eq:xxx:nene} guarantees that the user $i$'s  strategy  $\bs_i$ is feasible.

\subsubsection{Equilibrium Analysis}

We now analyze the NE of the Task Selection Game $\T$ \emph{without} the Taxation Mechanism, and show that the corresponding NE is often \emph{not} efficient.

We first show that the Task Selection Game $\T$ is a \emph{potential game} \cite{xxx-potential}.
A game is called an (exact) potential game, if there exists an (exact) \emph{potential function}, such that for any user, when changing his strategy, the change of his payoff is equivalent to that of the potential function.
Formally,

\begin{definition}[Potential Game \cite{xxx-potential}]\label{def:potential-game}
A game $\G = $ \\
$(\N, \{\S_i\}_{i\in\N}, \{\u_i\}_{i\in\N})$ is called a potential game, if it admits a potential function $\Phi(\bs)$ such that for every player $i\in \N$ and any two strategies $\bs_i,\bs_i' \subseteq \S_i $ of player $i$,
$$
\u_i (\bs_i, \bs_{-i} ) - \u_i (\bs_i', \bs_{-i} )
=
\Phi (\bs_i, \bs_{-i} ) - \Phi (\bs_i', \bs_{-i} ),
$$
under any strategy profile $\bs_{-i}$ of players other than $i$.
\end{definition}

\begin{lemma}\label{lemma:mcs:potential}
The Task Selection Game $\T$ is a potential game, with the following potential function  $\Phi(\bs)$:
\begin{equation}\label{eq:xxx:pf}
\begin{aligned}
 \Phi(\bs) =  \sum_{k \in \S} \sum_{m=1}^{M_k(\bs)} \frac{V_k   }{m}
  - \sum_{i \in \N } c_i^{\textsc{ex}} (\bs_i ) - \sum_{i \in \N } c_i^{\textsc{tr}} (\bs_i ),
% - \sum_{i \in \N } \sum_{k \in \bs_i } C_{i, k}
%  \\
%  &- \sum_{i \in \N }  \sum_{j = 1}^{ |\bs_i|  } D({k_i^{j-1}}, {k_i^{j}}) \cdot \widetilde{C}_{i}  ,
\end{aligned}
\end{equation}
where $M_k(\bs)$ is defined in \eqref{eq:xxx:mk}, i.e., the total number of users executing task $k$ under the strategy profile $\bs$.
\end{lemma}

\input{app-proof-mcs1}


An appealing property of a potential game is that it
always admits an NE. In addition, any strategy profile $\bs^*$ that maximizes the potential function $\Phi(\bs)$ is an NE. Therefore,

\begin{lemma}\label{lemma:mcs:NE}
The Task Selection Game $\T$ has at least one NE outcome $\bs^* \eq (\bs_1^*,\cdots,\bs_N^*)$, which is  given by
\begin{equation}\label{eq:xxx:NE}
\begin{aligned}
 \bs^* \eq  \arg \max_{\bs} &\  \  \Phi(\bs)
 \\
% \textstyle s.t. & \textstyle  \ \sum_{k \in \bs_i} c_{i,k} \leq C_i , \ \forall i\in \N,
   s.t.\  & \bs_i \mbox{ satisfies \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3}}, \ \forall i\in \N.
\end{aligned}
\end{equation}
where $\Phi(\bs)$ is the potential function defined in \eqref{eq:xxx:pf}.
\end{lemma}

\input{app-proof-mcs2}



Next we show that the NE of the Task Selection Game $\T$,  especially the one given by \eqref{eq:xxx:NE}, is often \emph{not} efficient.
Specifically, a strategy profile $\bs^\circ$ is socially efficient, if it maximizes the following social welfare:
\begin{equation}\label{eq:xxx:sw}
\W(\bs) = \sum_{k \in \S} V_k  \cdot \big( \mathbf{1}_{ M_k(\bs) \geq 1 } \big)
 - \sum_{i \in \N } \big( c_i^{\textsc{ex}} (\bs_i ) + c_i^{\textsc{tr}} (\bs_i ) \big) ,
\end{equation}
where $\mathbf{1}_{ M_k(\bs) \geq 1 } = 1$ if $M_k(\bs) \geq 1$, and $0$ otherwise. The first term denotes the total reward collected by all users, where the reward $V_k$ of a task $k$ is collected if at least one user chooses to execute the task (i.e., $M_k(\bs) \geq 1$).
The second term denotes the total cost incurred on all users.
Formally, the socially efficient solution $\bs^\circ$ is given by:
\begin{equation}\label{eq:xxx:soooo}
\begin{aligned}
 \bs^\circ \eq  \arg \max_{\bs} &\  \  \W(\bs)
 \\
% \textstyle s.t. & \textstyle  \ \sum_{k \in \bs_i} c_{i,k} \leq C_i , \ \forall i\in \N,
   s.t.\  & \bs_i \mbox{ satisfies \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3}}, \ \forall i\in \N.
\end{aligned}
\end{equation}

By comparing  $\W(\bs) $ in \eqref{eq:xxx:sw}
and 
 $ \Phi(\bs)$ in \eqref{eq:xxx:pf}, we can see that both functions have the similar structure, except the 
coefficients for $ V_k, k\in \S $. In particular, we have: 
%$$
%%\sum_{m=1}^{M_k(\bs)} \frac{1}{m} \geq  \big( \mathbf{1}_{ M_k(\bs) \geq 1 } \big),
% \sum_{k \in \S} V_k   \cdot  \sum_{m=1}^{M_k(\bs)} \frac{1 }{m}
% \geq \sum_{k \in \S} V_k  \cdot \big( \mathbf{1}_{ M_k(\bs) \geq 1 } \big),
%\quad \forall k\in\S,
%$$
$$ 
\sum_{m=1}^{M_k(\bs)} \frac{1  }{m}
 \geq   \mathbf{1}_{( M_k(\bs) \geq 1 )}, 
$$
where the equality holds only when $M_k(\bs) = 1$ or $0$.
Namely, the coefficient for each $ V_k$  in $ \Phi(\bs) $ is larger than that in $\W(\bs) $. 
This implies that the task selections at the NE, especially that resulting from  \eqref{eq:xxx:NE}, are more aggressive, comparing with those at the SE resulting from maximizing $ \W(\bs) $.

To illustrate this, we provide a simple example with one task and two users. Suppose that the reward of the task is $10$, the travelling costs of both users are zero, and the sensing costs of users are $4.8$ and $4.9$, respectively.
The SE outcome is: only user 1 chooses to execute the task, leading to a social welfare of $10-4.8 = 5.2$.
Under the NE, however, both users choose to execute the task (as both can achieve a positive payoff even if they share the reward), leading to a social welfare of $10-4.8-4.9 = 0.3$, a decrease of $1700\%$ comparing with that at the SE !


\subsubsection{\textbf{Implementation of Taxation Mechanism}}


Now we implement the Taxation Mechanism in the Task Selection Game $\T$ to induce the efficient and fair equilibrium.

For ease of illustration, we set  $\bg = 1$ (i.e., strictly budget balance) and $\ex_i = 0, \forall i\in \N$ (i.e., zero tax exemptions for all users, leading to the Max-min fairness by Lemma \ref{lemma:fair1}).
According to Theorem \ref{thm:efficiency}, the efficient flat taxing rule is:
\begin{equation}
\r_i = \r = \frac{N-1}{N}, \quad \forall i \in \N.
\end{equation}

With the above taxing rule, the new payoff of each user $i\in \N$  in the Taxation Version of the game $\T$, according to  \eqref{eq:xxx}, can be computed as follows:
\begin{equation}\label{eq:xxx:payoff-tax}
\begin{aligned}
 \ux_i (\bs) &   =  \left(1 - \frac{N-1}{N}\right) \u_i(\bs) + \frac{N-1}{N}   \frac{1}{N-1}   \sum_{j\neq i}\u_j(\bs)
 \\
% &   = \frac{ 1}{N}  \cdot \u_i(\bs ) + \frac{ 1}{N}  \cdot \sum_{j \neq i } \u_j(\bs )
% \\
 &     =\frac{ 1}{N} \cdot \sum_{j \in \N } \left(   \sum_{k \in \bs_j} \frac{V_k}{M_k (\bs)} - c_j^{\textsc{ex}} (\bs_j ) - c_j^{\textsc{tr}} (\bs_j ) \right).
\end{aligned}
\end{equation}
Recall that $M_k (\bs) =   \sum_{i \in \N} \mathbf{1}_{(k \in \bs_i)}
$ according to \eqref{eq:xxx:mk}.
Substitute $M_k (\bs) $ into \eqref{eq:xxx:payoff-tax}, we have:
$$
 \sum_{j \in \N }  \sum_{k \in \bs_j} \frac{V_k}{M_k (\bs)}
 =  \sum_{k \in \S} V_k  \cdot \big( \mathbf{1}_{ M_k(\bs) \geq 1 } \big).
 $$
 Thus, the new payoff of user $i$ in  \eqref{eq:xxx:payoff-tax} can be written as
$$
 \ux_i (\bs) = \frac{1}{N} \cdot \W(\bs) ,
$$
where $\W(\bs)$ is the social welfare defined in \eqref{eq:xxx:sw}.
This means that the individual objective of each user is aligned with the social objective.
Hence, the socially efficient outcome $\bs^\circ$ that maximizes the social welfare $\W(\bs)$ is an equilibrium of the Taxation Version of game $\T$. Formally,


\begin{lemma}\label{lemma:mcs:tax}
For the Task Selection Game $\T$,
we can achieve at least one efficient equilibrium, i.e., $\bs^\circ$, by implementing the Taxation Mechanism with the taxing rule:
$$
\r_i = \frac{N-1}{N},\ \ \ex_i = 0,\quad \forall i\in\N.
$$
At this equilibrium $\bs^\circ$, all users share the  (maximum) social welfare equally (i.e., Max-min fairness).
\end{lemma}

\input{app-proof-mcs3}

%
%\comm{The setting of one task seems to be too simple. A reader can easily argue that the result is not typical, and having more tasks might have completely different results. }


\subsubsection{Simulation Results}
\revvm{Now we provide simulation results to illustrate the social welfare gain achieved from the proposed Taxation Mechanism (with the efficient taxing rule).
We consider an MCS scenario with 10 tasks and $N\in\{2, 4, \cdots, 20\}$ users in the simulations, where
the execution cost of each user is randomly and uniformly selected from $[0,1]$,
and the reward $V_k$ of each task $k$ changes from $0.2$ to $1$ with a stepsize of $0.2$.
In order to obtain more useful engineering insights, we assume that (i) each task is valid in the whole time period, and (ii) each user has a zero travelling cost. Simulation results for the more general scenarios can be found in our online technical report \cite{report}.}

%\comm{The current simulation results are applicable for multi-task scenarios. Due to time limit, I will perform the simulations for the more general scenarios later.}

\begin{figure}
	\centering
\includegraphics[width=3in]{Figures/simu-1}
\\
\vspace{-3mm}
Reward -- $V_k$
\\
	\caption{Social Welfare under SE and NE.}
\label{fig:simu-1}
\vspace{-4mm}
\end{figure}

Figure \ref{fig:simu-1} illustrates the normalized social welfare under the NE (the hollow bars with the red borders) and under the SE (the blue bars).
Each bar group denotes the simulation results under a particular task reward, and different bars in the same group correspond to different numbers of users.
Note that the SE is induced by our proposed Taxation Mechanism (with the efficient taxing rule), while the NE is achieved in the original game situation without the Taxation Mechanism.
Hence, the social welfare gap between the SE and the NE can be viewed as the social welfare gain achieved by our proposed Taxation Mechanism.
From Figure \ref{fig:simu-1}, we can see that such a social welfare gain increases from $20\% $ to $ 80\%$ (on average), when the user number increases from $2$ to $20$.
%task reward changes from $0.2$ to $1$.
From Figure \ref{fig:simu-1}, we further have the following observations.
\begin{enumerate}
  \item \emph{The social welfare under SE increases with the number of users (for any possible task reward).}
      The reason is that with more users, it is more likely to choose  users with smaller costs to execute the tasks.
  \item \emph{When the task reward is small (e.g., $V_k = 0.2$), the social welfare under NE   increases with the number of users.}
      The reason is similar as point (1): with more users, it is more likely to choose users with  smaller costs to execute  the tasks.
  \item  \emph{When the task reward is medium (e.g., $V_k \in [0.4,0.8]$), however, the social welfare under NE first increases and then decreases with the number of users.}
      This is because when there are few users, with more users it is more likely to choose users with  smaller costs to execute the tasks; while when there are sufficient users, with more users it is more likely to choose  multiple users to execute the same task, which will reduce the social welfare.
  \item  \emph{When the task reward is large (e.g., $V_k  = 1$), the social welfare under NE decreases with the number of users.}
      The reason is that with more users it is more likely to choose  multiple users to execute the same task, which will reduce the social welfare.
\end{enumerate}

\revvm{Figure \ref{fig:simu-1} implies that with our proposed Taxation Mechanism (that leads to the  SE), it is always beneficial to involve more users in the system; while without the proposed Taxation Mechanism (leading to the NE), it may not be beneficial to involve more users, due to the increased competition among users.
\emph{This implies that our proposed Taxation Mechanism can reconcile the competition among users and align the individual objectives with the social objective, hence reach the desired efficient equilibrium}.}
%This implies that our proposed Taxation Mechanism can align the individual objectives with the social objective, hence reach the desired efficient equilibrium.

%\comm{We can show other performance criterions, e.g., fairness and platform budget, but the results are quite intuitive (i.e., same as the analytical results).
%Moreover, the comparison of the proposed mechanism and the existing Altruistic mechanism is also quite intuitive (i.e., same as the analytical results).}







==> section4-app-MCWA.tex <==

\subsection{Application II: Mobile Crowdsourced Wireless Access}

Mobile Crowdsourced Wireless Access (MCWA) enables nearby mobile devices to form a cooperative group (via D2D communication technology such as WiFi or Bluetooth) and  crowdsource their wireless access channels and resources
for the  cooperative data downloading and uploading \cite{yyy-1}.
Such a novel networking scheme reconciles the mismatch between mobile users' data demands and their wireless access capacities,
hence can achieve a more efficiently utilization of wireless resources.

In this application, we will formulate a \emph{Channel Selection Game} for a general MCWA model similar as that in \cite{yyy-1}, 
and show how to implement the Taxation Mechanism in this game, and how the Taxation Mechanism will steer the
results of the Channel Selection Game to a desirable one.
Due to space limit, we leave the detailed discussion in our online technical report \cite{report}.

%\input{app-mcwa}


==> section4-applications.tex <==


\section{Applications}\label{sec:applications}

In this section, we illustrate the proposed mechanism through the game of Prisoners' Dilemma, and implement it in two wireless networking applications:  \emph{Mobile Crowd Sensing} and \emph{Mobile Crowdsourced Wireless Access}.
%we implement the proposed Taxation Mechanism, together with the derived taxing rule, in two wireless networking applications: Mobile Crowd Sensing (MCS) and Mobile Crowdsourced Wireless Access (MCWA), both are important research topics for the future wireless networks with  human-in-the-loop (HITL) \cite{hitl}.
The main purpose is to show how to implement the Taxation Mechanism in a real game.
In particular, we will illustrate how to interpret the tax, how to impose the tax, how to manipulate the tax, and how to redistribute the tax, in a practical scenario.
%Due to space limit, we leave most of the detailed analysis in our online technical report \cite{report}.
%We have also applied our mechanism in the design of \emph{Mobile Crowdsourced Wireless Access (MCWA)} schemes.
%Due to space limit, we leave the discussion regarding MCWA in our online technical report \cite{report}.

\subsection{An Illustrative Example}

Before implementing the Taxation Mechanism in real applications, we first provide an illustrative example regarding the implementation of the mechanism in the Prisoner's Dilemma   \cite{game-theory1994}, a widely-used game example in game theory.

In the Prisoner's Dilemma game, two players make choices with strategic inter-dependence.
Each player can choose the strategy ``Cooperate'' or ``Defect''.
Hence, there are four possible strategy profiles.
The payoffs of players under four strategy profiles are illustrated in
Table \ref{tbl:1}, where each row (or column) denotes the choice of player 1 (or 2), and the numbers in each cell denote the payoffs of both players under a particular strategy profile.
We can see that the unique NE of this game is (Defect, Defect), where both players choose ``Defect''.
However, the unique SE is (Cooperate, Cooperate), where both players should choose ``Cooperate''.
%which is inefficient from the social perspective.
%That is, the social efficient outcome is to choose the Cooperate for both players.

\begin{table} [t]
\centering
\caption{The Prisoner's Dilemma Game}\label{tbl:1}
	\begin{tabular}{|c|c|c|}
	\hline
	           & Cooperate &	Defect
	 \\
	 \hline
	 Cooperate	& ~~~~~~~~$(2 ,\ 2 )$ ~~~~~~ &~~~~~~~ $(0 ,\ 3 )~~~~~~$
	 \\
	 \hline
	 Defect & ~$(3 ,\ 0 )$ &~ $\mathbf{(1 ,\ 1 )}$
	 \\
	 \hline
	\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{A Taxation Version of The Prisoner's Dilemma Game with $\r_1 = \r_2 = 0.5$ and $\ex_1= \ex_2 = 0$}\label{tbl:2}
	\begin{tabular}{|c|c|c|}
	\hline
	 & Cooperate &	Defect
	 \\
	 \hline
	 Cooperate	& $\mathbf{(2 ,\ 2  )}$ & $( {1.5},\  {1.5})$
	 \\
	 \hline
	 Defect &  $(  {1.5},\  {1.5})$ & $(1 ,\ 1 )$
	 \\
	 \hline
	\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{A Taxation Version of The Prisoner's Dilemma Game with $\r_1 = \r_2 = 0.5$ and $\ex_1= 0, \ex_2 = 1$}\label{tbl:3}
	\begin{tabular}{|c|c|c|}
	\hline
	 & Cooperate &	Defect
	 \\
	 \hline
	 Cooperate	& $\mathbf{(1.5,\ 2.5 )}$ & $( {2},\ 1)$
	 \\
	 \hline
	 Defect &  $(1,\ 2)$ & $(  {0.5},\ 1.5)$
	 \\
	 \hline
	\end{tabular}
\end{table}


Now we implement the Taxation Mechanism to the Prisoner's Dilemma game.
For ease of illustration, we assume that $\bg = 1$ (strictly budget balance).
According to Theorem \ref{thm:efficiency}, the efficient taxing rule is: $\r = \frac{N-1}{N} = 0.5$.
Note that the tax exemptions will not affect the efficiency.
We take two different tax exemptions as illustrative examples.
First, the tax exemptions are $0$ for both players. In this case, the new payoffs of players (after taxation) can be computed by \eqref{eq:xxx}, and illustrated in Table \ref{tbl:2}.
Second, the tax exemption is $0$ for one player and $1$ for another player.
In this case, the new payoffs of players are illustrated in Table \ref{tbl:3}.
We can see that in both cases, the unique NE  of the new Taxation Version game is (Cooperate, Cooperate), which is an efficient outcome of both the new and  original  game.

In what follows, we will implement the Taxation Mechanism  in two wireless networking applications: Mobile Crowd Sensing and Mobile Crowdsourced Wireless Access.


\input{section4-app-MCS}


\input{section4-app-MCWA}

